Video-Text Pre-training with Learned Regions

Video-Text pre-training aims at learning transferable representations from large-scale video-text pairs via aligning the semantics between visual and textual information. State-of-the-art approaches extract visual features from raw pixels in an end-to-end fashion. However, these methods operate at frame-level directly and thus overlook the spatio-temporal structure of objects in video, which yet has a strong synergy with nouns in textual descriptions. In this work, we propose a simple yet effective module for video-text representation learning, namely RegionLearner, which can take into account the structure of objects during pre-training on large-scale video-text pairs. Given a video, our module (1) first quantizes visual features into semantic clusters, then (2) generates learnable masks and uses them to aggregate the features belonging to the same semantic region, and finally (3) models the interactions between different aggregated regions. In contrast to using off-the-shelf object detectors, our proposed module does not require explicit supervision and is much more computationally efficient. We pre-train the proposed approach on the public WebVid2M and CC3M datasets. Extensive evaluations on four downstream video-text retrieval benchmarks clearly demonstrate the effectiveness of our RegionLearner. The code will be available at https://github.com/ruiyan1995/Region_Learner.

==> mov2.tex <==

\begin{figure}[t]
  \centering
%   \fbox{\rule{0pt}{4in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1\linewidth]{mov2_tmp.pdf}
   \caption{Different granularity of video features used to visual-text alignment.}
   \label{fig:motivation}
\end{figure}

==> tab5.tex <==

\begin{table*}[!t]
  \centering
  \begin{tabular}{@{}lccc|cccc|cccc@{}}
    \toprule
    &&&&\multicolumn{4}{c}{Text $\Longrightarrow$ Video} &\multicolumn{4}{|c}{Video $\Longrightarrow$ Text}\\
    Method & E2E & PT dataset & \#pairs & R@1 &R@5 &R@10 & MedR & R@1 &R@5 &R@10 & MedR\\
    \midrule
    JSFusion & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    HT MIL-NCE & x &&&&&&&&&&\\
    Ours & x &&&&&&&&&&\\
    \bottomrule
  \end{tabular}
  \caption{Comparison to state-of-the-art results on MSR-VTT for text-to-video retrieval.}
  \label{tab:example}
\end{table*}

==> tab_depth_STATT.tex <==

\begin{table}[!t]
  \centering
  \begin{tabular}{@{}r|rrrr@{}}
    \toprule
    \multirow{2}*{depth} &\multicolumn{4}{c}{Text $\Longrightarrow$ Video}\\
      & R@1 &R@5 &R@10 & MedR\\
    \midrule
    1 &$\mathbf{34.3}$ &$60.2$ &$72.0$ &$\textbf{3.0}$\\
    2 &$33.1$ &$59.9$ &$70.8$ &$\textbf{3.0}$\\
    4 &$33.1$ &$\mathbf{61.0}$ &$\textbf{72.2}$ &$\textbf{3.0}$\\
    6 &$33.3$ &$60.5$ &$71.1$ &$\textbf{3.0}$\\
    8 &$32.4$ &$59.2$ &$70.4$ &$\textbf{3.0}$\\
    \bottomrule
  \end{tabular}
  \caption{Effect of depth of spatio-temporal interaction layer on MSRVTT 1K-A.}
  \label{tab:num_regions}
\end{table}

==> tab_numregion.tex <==

\begin{table}[!t]
  \centering
  \begin{tabular}{@{}l|llll@{}}
    \toprule
    \multirow{2}*{Method} &\multicolumn{4}{c}{Text $\Longrightarrow$ Video}\\
      & R@1 &R@5 &R@10 & MedR\\
    \midrule
    1 &$31.2$ &$-$ &$-$ &$-$\\
    2 &$31.2$ &$-$ &$-$ &$-$\\
    4 &$33.1$ &$-$ &$-$ &$-$\\
    8 &$33.5$ &$-$ &$-$ &$-$\\
    16 &$32.6$ &$-$ &$-$ &$-$\\
    32 &$32.2$ &$-$ &$-$ &$-$\\
    64 &$32.6$ &$-$ &$-$ &$-$\\
    \bottomrule
  \end{tabular}
  \caption{Effect of number of regions on MSRVTT 1K-A.}
  \label{tab:num_regions}
\end{table}
